A novel multimodal fusion network based on a joint coding model for lane line segmentation

There has recently been growing interest in utilizing multimodal sensors to achieve robust lane line segmentation. In this paper, we introduce a novel multimodal fusion architecture from an information theory perspective, and demonstrate its practical utility using Light Detection and Ranging (LiDAR) camera fusion networks. In particular, we develop, for the first time, a multimodal fusion network as a joint coding model, where each single node, layer, and pipeline is represented as a channel. The forward propagation is thus equal to the information transmission in the channels. Then, we can qualitatively and quantitatively analyze the effect of different fusion approaches. We argue the optimal fusion architecture is related to the essential capacity and its allocation based on the source and channel. To test this multimodal fusion hypothesis, we progressively determine a series of multimodal models based on the proposed fusion methods and evaluate them on the KITTI and the A2D2 datasets. Our optimal fusion network achieves 85%+ lane line accuracy and 98.7%+ overall. The performance gap among the models will inform continuing future research into development of optimal fusion algorithms for the deep multimodal learning community.

==> bbm/README <==
Copyright 1993 Gilles F. Robert.
You may freely use, modify and/or distribute this file.
This statement added 2008/11/14 by Clea F. Rees on the basis of the email exchange archived at http://lists.debian.org/debian-tex-maint/2008/05/msg00040.html.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A mathematician often needs special symbols to designate sets such as the
integers, the reals etc..

For the time being, the only fonts providing these special symbols have been:
 - the AMS fonts msbm (older version msym), which are intended for use with
Times and aren't truly what a mathematician expects (the stress is on both
stems instead of being on only the left one).
 - Alan Jeffrey's bbold fonts, which are sans-serif ones, with (almost) no
possibility of design variations for, say, a bold variant.
That was all, and in particular nothing for use with Computer Modern.

I was already working at that time on the project of changing the codes of
romanu.mf, romanl.mf and other files to add a 'Blackboard' variant to
Computer Modern.

                YOU HAVE IT ALL THERE !!!

The whole package contains five 'main' files:
 - blbbase.mf (the 'base') contains the supplementary definitions needed
for double stems etc..
 - blbord.mf (the 'driver') is fairly simple and only makes the necessary
calls.
 - blbordu.mf (based on romanu.mf): programs for uppercase letters.
 - blbordl.mf (based on romanl.mf): programs for lowercase letters.
 - blbordsp.mf (based on romand.mf and punct.mf): programs for the digits~1
and~2 and for parentheses and brackets.

There is also a whole lot of parameter files that are (almost) the same as
those provided by DEK.

For most of them, the only differences are
- change 'cmbase' for 'blbbase' on line~2
- change 'generate roman' for 'generate blbord' on last line
- add two extra parameters (interspace# and cap_interspace#).

A LaTeX(2e) package written by Torsten Hilbrich for using these fonts is also 
available nearby, exactly in ctan/macros/latex/contrib/supported/bbm/

I sincerely hope you'll enjoy using these fonts; if you get into problems
while using them, I should be reachable at

 _ _       Gilles F. ROBERT
|          Unit\'e de Math\'ematiques Pures et Appliqu\'ees
|  _ _ _   \'Ecole Normale Sup\'erieure
|   |   |  46, All\'ee d'Italie
|_ _|_ _|  69364 Lyon Cedex (FRANCE)
    |  \
    |   \  e-mail : gfrobert@umpa.ens-lyon.fr

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> bbm/test.tex <==
% Copyright 1993 Gilles F. Robert.
% You may freely use, modify and/or distribute this file.
% This statement added 2008/11/14 by Clea F. Rees on the basis of the email exchange archived at http://lists.debian.org/debian-tex-maint/2008/05/msg00040.html.
%
\let\noinit!\input testfont
\def\fontname{bbm17 }\startfont\table
\def\fontname{bbm12 }\startfont\table
\eject
\def\fontname{bbm10 }\startfont\table
\def\fontname{bbm9 }\startfont\table
\eject
\def\fontname{bbm8 }\startfont\table
\def\fontname{bbm7 }\startfont\table
\eject
\def\fontname{bbm6 }\startfont\table
\def\fontname{bbm5 }\startfont\table
\eject
\def\fontname{bbmsl12 }\startfont\table
\def\fontname{bbmsl10 }\startfont\table
\eject
\def\fontname{bbmsl9 }\startfont\table
\def\fontname{bbmsl8 }\startfont\table
\eject
\def\fontname{bbmbx12 }\startfont\table
\def\fontname{bbmbx10 }\startfont\table
\eject
\def\fontname{bbmbx9 }\startfont\table
\def\fontname{bbmbx8 }\startfont\table
\eject
\def\fontname{bbmbx7 }\startfont\table
\def\fontname{bbmbx6 }\startfont\table
\eject
\def\fontname{bbmbx5 }\startfont\table
\def\fontname{bbmbxsl10 }\startfont\table
\eject
\def\fontname{bbmss17 }\startfont\table
\def\fontname{bbmss12 }\startfont\table
\eject
\def\fontname{bbmss10 }\startfont\table
\def\fontname{bbmss9 }\startfont\table
\eject
\def\fontname{bbmss8 }\startfont\table
\def\fontname{bbmssq8 }\startfont\table
\eject
\def\fontname{bbmssi17 }\startfont\table
\def\fontname{bbmssi12 }\startfont\table
\eject
\def\fontname{bbmssi10 }\startfont\table
\def\fontname{bbmssi9 }\startfont\table
\eject
\def\fontname{bbmssi8 }\startfont\table
\def\fontname{bbmssqi8 }\startfont\table
\eject
\def\fontname{bbmssbx10 }\startfont\table
\def\fontname{bbmssdc10 }\startfont\table
\eject
\def\fontname{bbmtt12 }\startfont\table
\def\fontname{bbmtt10 }\startfont\table
\eject
\def\fontname{bbmtt9 }\startfont\table
\def\fontname{bbmtt8 }\startfont\table
\eject
\def\fontname{bbmsltt10 }\startfont\table
\def\fontname{bbmvtt10 }\startfont\table
\eject
\def\fontname{bbmb10 }\startfont\table
\def\fontname{bbmfib8 }\startfont\table
\eject
\def\fontname{bbmdunh10 }\startfont\table
\bye

